Entity-Aware Language Model as an Unsupervised Reranker

In language modeling, it is difficult to incorporate entity relationships from a knowledge-base. One solution is to use a reranker trained with global features, in which global features are derived from n-best lists. However, training such a reranker requires manually annotated n-best lists, which is expensive to obtain. We propose a method based on the contrastive estimation method that alleviates the need for such data. Experiments in the music domain demonstrate that global features, as well as features extracted from an external knowledge-base, can be incorporated into our reranker. Our final model, a simple ensemble of a language model and reranker, achieves a 0.44\% absolute word error rate improvement over an LSTM language model on the blind test data.

==> algo.tex <==
\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LState{\State \algbackskip}%
\makeatother

\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LComment{\Comment \algbackskip}%
\makeatother

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{figure}[t!]
\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\vspace{0.2cm}
%\noindent\rule{0.5\textwidth}{0.4pt}
\begin{algorithmic}[0]
\small
 \LState {{\bf Inputs: }{1) Training data ${\cal S} = \{S^{(1)}, \ldots, S^{(m)}\}$; and 2) A phonetic similarity function $\psi(w, w')$ for words $w$ and $w'$.}}
\vspace{0.2cm}
\LState{\bf Algorithm:}
\State ${\cal V }$: List of words derived from ${\cal S}$.
\State Train ngram language model $\theta_{ngram}$ on ${\cal S}$.
\State ${\cal D} = \{ \}$
\For {$i$ = 1 to $m$}
\State L = \{\}
\For {$j$ = 1 to $30$}
\State $x= S^{(i)}$
\State Sample $r \sim unif(\{1,2,3\})$
\For {$k$ = 1 to $r$}
\State Sample $z_k \sim unif(\{1, \ldots, |x|\})$
\State Sample $z \in {\cal V} \sim \psi(z, x_{z_k})$ 
\State Set $x_{z_k} = z$
\EndFor
\State $L = L \cup X $
\EndFor
\State $L'$ = top $5$ sentences in $L$ according to $\theta_{ngram}$.
\State $D = D \cup L'$
\EndFor
\vspace{0.2cm}
\LState {{\bf Output: } Top 1M n-best lists in $D$ according to the average ngram probability in the n-best list.}
\end{algorithmic}

\vspace{0.2cm}

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\caption{The algorithm for creating training data for the noise contrastive estimation training.}\label{algo_neg}

\end{figure}

